Strategic (Timed) Computation Tree Logic

We define extensions of CTL and TCTL with strategic operators, called Strategic CTL (SCTL) and Strategic TCTL (STCTL), respectively. For each of the above logics we give a synchronous and asynchronous semantics, i.e., STCTL is interpreted over networks of extended Timed Automata (TA) that either make synchronous moves or synchronise via joint actions. We consider several semantics regarding information: imperfect (i) and perfect (I), and recall: imperfect (r) and perfect (R). We prove that SCTL is more expressive than ATL for all semantics, and this holds for the timed versions as well. Moreover, the model checking problem for SCTL[ir] is of the same complexity as for ATL[ir], the model checking problem for STCTL[ir] is of the same complexity as for TCTL, while for STCTL[iR] it is undecidable as for ATL[iR]. The above results suggest to use SCTL[ir] and STCTL[ir] in practical applications. Therefore, we use the tool IMITATOR to support model checking of STCTL[ir].

==> figures/tikzTemplates.tex <==
%!TEX root=../report.tex

\newcommand{\leafAgent}[4][(0,0)]{%
	\node[state,initial] (l0) at #1 {$\loc_0$};
	\node[state,right of=l0] (l1) {$\loc_1$};
	\node[state,below of=l1, node distance=1cm] (l'1) {$\loc'_1$};
	\draw (l0) -- node[above] (action) {$#2$} (l1);
	\ifstrempty{#4}{}{
		\node[above of=action,node distance=0.4cm,
			text=colorAttribute] (time) {$#4$};
	}
	\ifstrempty{#3}{}{
		\node[above of=time,node distance=0.4cm,
			text=colorAttribute] (cost) {$#3$};
	}
	\draw[sync] (l1) to [loop right]
		node[above,yshift=0.1cm] {$\styleSync{\send{}#2\_\ok}$} (l1);
	\draw[sync] (l0) --
		node[below,sloped] {$\styleSync{\send{}#2\_\nok}$} (l'1);
	\draw[sync] (l'1) to [loop right]
		node[below,yshift=-1.5mm,pos=0.5] {$\styleSync{\send{}#2\_\nok}$} (l'1);
}


\newcommand{\andAgent}[6][(0,0)]{%
	\node[state,initial] (l0) at #1 {$\loc_0$};
	\node[state,right of=l0] (l1) {$\loc_1$};
	\node[state,right of=l1] (l2) {$\loc_2$};
	\node[state,right of=l2] (l4) {$\loc_{#2}$};
	\node[state,below of=l1] (l'1) {$\loc'_1$};

	\draw[sync] (l0) --
		node[above] {$\styleSync{\receive{}#3\_\ok}$} (l1);
	\draw[sync] (l1) --
		node[above] {$\styleSync{\receive{}#4\_\ok}$} (l2);

	\draw (l2) -- node[above] (action) {$#2$} (l4);
	\ifstrempty{#6}{}{
		\node[above of=action,node distance=0.4cm,
			text=colorAttribute] (time) {$#6$};
	}
	\ifstrempty{#5}{}{
		\node[above of=time,node distance=0.4cm,
			text=colorAttribute] (cost) {$#5$};
	}
	\draw[sync] (l4) to [loop right]
		node[above,yshift=0.1cm] {$\styleSync{\send{}#2\_\ok}$} (l4);

	\draw[sync] (l0) --
		node[above,sloped] {$\styleSync{\receive{}#3\_\nok}$} (l'1);
	\draw[sync] (l0) to [bend right=30]
		node[above,sloped] {$\styleSync{\receive{}#4\_\nok}$} (l'1);

	\draw[sync] (l'1) to [loop right]
		node[below,yshift=-1.5mm,pos=0.5] {$\styleSync{\send{}#2\_\nok}$} (l'1);
}


\newcommand{\orAgent}[8][(0,0)]{%
	\node[state,initial] (l0) at #1 {$\loc_0$};
	\node[state,right of=l0] (l1) {$\loc_1$};
	\node[state,right of=l1] (l2) {$\loc_{#2}$};
	\node[state,below of=l1] (l'1) {$\loc'_1$};
	\node[state,right of=l'1] (l'2) {$\loc'_2$};

	\draw[sync] (l0) to [bend left]
		node[above] (action1) {$\styleSync{\receive{}#3\_\ok}$} (l1);
	\ifstrempty{#6}{}{
		\node[above of=action1,node distance=0.4cm,
			text=colorAttribute] (time1) {$#6$};
	}
	\ifstrempty{#5}{}{
		\node[above of=time1,node distance=0.4cm,
			text=colorAttribute] (cost1) {$#5$};
	}
	\draw[sync] (l0) to [bend right]
		node[below] (action2) {$\styleSync{\receive{}#4\_\ok}$} (l1);
	\ifstrempty{#8}{}{
		\node[below of=action2,node distance=0.4cm,
			text=colorAttribute] (time2) {$#8$};
	}
	\ifstrempty{#7}{}{
		\node[below of=time2,node distance=0.4cm,
			text=colorAttribute] (cost2) {$#7$};
	}
	\draw (l1) -- node[above] {$#2$} (l2);
	\draw[sync] (l2) to [loop right]
		node[above,yshift=0.1cm] {$\styleSync{\send{}#2\_\ok}$} (l2);

	\draw[sync] (l0) to [bend right=30] node[below,sloped,very near end]
		{$\styleSync{\hspace{-3.5em}\receive{}#3\_\nok}$} (l'1);
	\draw[sync] (l'1) -- node[above]
		{$\styleSync{\receive{}#4\_\nok}$} (l'2);
	\draw[sync] (l'2) to [loop right]
		node[below,yshift=-1.5mm,pos=0.5] {$\styleSync{\send{}#2\_\nok}$} (l'2);
}


\newcommand{\nandAgent}[7][(0,0)]{%
	\node[state,initial] (l0) at #1 {$\loc_0$};
	\node[state,right of=l0] (l1) {$\loc_1$};
	\node[state,below of=l1] (l'1) {$\loc'_1$};
	\node[state,right of=l1] (l2) {$\loc_2$};
	\node[state,right of=l2] (lA) {$\loc_{#2}$};

	\draw[sync] (l0) --
		node[above] {$\styleSync{\receive{}#3\_\ok}$} (l1);
	\draw[sync] (l1) --
		node[above] {$\styleSync{\receive{}#4\_\nok}$} (l2);

	\draw[sync] (l0) -- node[above,sloped]
		{$\styleSync{\receive{}#3\_\nok}$} (l'1);
	\draw[sync] (l0) to [bend right] node[below,sloped]
		{$\styleSync{\receive{}#4\_\ok}$} (l'1);
	\draw (l2) -- node[above] (action) {$#2$} (lA);
	\ifstrempty{#5}{}{
		\node[below of=action,node distance=0.8cm,
			text=colorAttribute] (cost) {$#5$};
	}
	\ifstrempty{#6}{}{
		\node[below of=cost,node distance=0.4cm,
			text=colorAttribute] (time) {$#6$};
	}
	\ifstrempty{#7}{}{
		\node[above of=action,node distance=0.4cm,
			text=RedOrange] (condition) {$#7$};
	}
	\draw[sync] (lA) to [loop right]
		node[above,yshift=0.1cm] {$\styleSync{\send{}#2\_\ok}$} (lA);
	\draw[sync] (l'1) to [loop right]
		node[below,yshift=-1.5mm,pos=0.5] {$\styleSync{\send{}#2\_\nok}$} (l'1);
}

\newcommand{\sandAgent}[6][(0,0)]{%
	\node[state,initial] (l0) at #1 {$\loc_0$};
	\node[state,right of=l0] (l1) {$\loc_1$};
	\node[state,below of=l1,node distance=2cm] (l'1) {$\loc'_1$};
	\node[state,right of=l1] (l2) {$\loc_2$};
	\node[state,right of=l2] (lA) {$\loc_{#2}$};

	\draw[sync] (l0) --
		node[above] {$\styleSync{\receive{}#3\_\ok}$} (l1);
	\draw[sync] (l1) --
		node[above] {$\styleSync{\receive{}#4\_\ok}$} (l2);
	\draw[sync] (l0) -- node[above,sloped]
		{$\styleSync{\receive{}#3\_\nok}$} (l'1);
	\draw[sync] (l1) to node[above,sloped]
		{$\styleSync{\receive{}#4\_\nok}$} (l'1);
	\draw (l2) -- node[above] (action) {$#2$} (lA);
	\ifstrempty{#6}{}{
		\node[above of=action,node distance=0.4cm,
			text=colorAttribute] (time) {$#6$};
	}
	\ifstrempty{#5}{}{
		\node[above of=time,node distance=0.4cm,
			text=colorAttribute] (cost) {$#5$};
	}
	\draw[sync] (lA) to [loop right]
		node[above,yshift=0.1cm] {$\styleSync{\send{}#2\_\ok}$} (lA);
	\draw[sync] (l'1) to [loop right]
		node[below,yshift=-1.5mm,pos=0.5] {$\styleSync{\send{}#2\_\nok}$} (l'1);
}

